Learning from MOM's principles: Le Cam's approach

We obtain estimation error rates for estimators obtained by aggregation of regularized median-of-means tests, following a construction of Le Cam. The results hold with exponentially large probability -- as in the gaussian framework with independent noise- under only weak moments assumptions on data and without assuming independence between noise and design. Any norm may be used for regularization. When it has some sparsity inducing power we recover sparse rates of convergence. The procedure is robust since a large part of data may be corrupted, these outliers have nothing to do with the oracle we want to reconstruct. Our general risk bound is of order \begin{equation*} \max\left(\mbox{minimax rate in the i.i.d. setup}, \frac{\text{number of outliers}}{\text{number of observations}}\right) \enspace. \end{equation*}In particular, the number of outliers may be as large as (number of data) $\times$(minimax rate) without affecting this rate. The other data do not have to be identically distributed but should only have equivalent $L^1$ and $L^2$ moments. For example, the minimax rate $s \log(ed/s)/N$ of recovery of a $s$-sparse vector in $\mathbb{R}^d$ is achieved with exponentially large probability by a median-of-means version of the LASSO when the noise has $q_0$ moments for some $q_0>2$, the entries of the design matrix should have $C_0\log(ed)$ moments and the dataset can be corrupted up to $C_1 s \log(ed/s)$ outliers.

==> commandes_guillaume.tex <==
\newcommand{\inr}[1]{\bigl< #1 \bigr>}

%\newcommand{\norm}[1]{\left\|#1\right\|}%
% j'ai enleve \left et \right pour eviter d'aboir des normes tres hautes
\newcommand{\norm}[1]{\left\|#1\right\|}%
\newcommand{\an}{{\mbox{ and }}}

\newcommand\set[2]{\{#1,\dots,#2\}}
\newcommand\und[2]{\underset{#2}{#1}\;}
\newcommand\undc[2]{{#1}_{#2}\;}
\newcommand\ove[2]{\overset{#2}{#1}\;}
\newcommand\ovec[2]{{#1}^{#2}\;}
\newcommand\undn{\und{\longrightarrow}{n\rightarrow +\infty}}
\newcommand\limn{\und{\lim}{n\rightarrow +\infty}}
\newcommand\limnps{\ove{\longrightarrow}{\rm p.s.}}
\newcommand{\pa}[1]{\left(#1\right)}
\newcommand{\cro}[1]{\left\{#1\right\}}
\newcommand{\Bi}[1]{\Big(#1\Big)}
\newcommand{\bi}[1]{\big(#1\big)}

\newcommand\qqua{\hspace*{1cm}}
\newcommand\eps{\epsilon}

\newcommand\ra{\rightarrow}
\newcommand\Ra{\Rightarrow}
\newcommand\Lra{\Leftrightarrow}
\newcommand\lra{\longrightarrow}
\newcommand\lin{\centerline{**********************}}
%\newcommand\to{\rightarrow}

%\DeclareMathOperator{\est}{{\hat f_{K,\lambda}}
\newcommand{\est}{{\hat f}_{K,\lambda}}%
\newcommand{\esti}{{\hat f}_{K}}
\newcommand{\eststar}{{\hat f}_{K^*,\lambda}}

\newcommand{\beginproof}{{\bf Proof. {\hspace{0.2cm}}}}
\def \endproof
{{\mbox{}\nolinebreak\hfill\rule{2mm}{2mm}\par\medbreak}}

%%%%%%%%%%%%%%%%%Operator
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\supp}{Supp}
\DeclareMathOperator{\limInf}{liminf}
\DeclareMathOperator{\limSup}{limsup}
\DeclareMathOperator{\pen}{pen}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator*{\rank}{rank}
%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand\limSupn{\und{\limSup}{n\rightarrow +\infty}}
\newcommand\limInfn{\und{\limInf}{n\rightarrow +\infty}}
\newcommand{\coF}{{\rm conv}(F)}
\newcommand{\ERM}{\hat f_n^{ERM}}
\newcommand{\kerA}{{\rm Ker}(A)}
\newcommand{\design}{\mathbb{X}}
\newcommand{\hbeta}{{\boldsymbol{\hat\beta}}}

%\let\leq\leqslant
%\let\geq\geqslant
%\let\vec\overrightarrow
\def\ds1{\textrm{1\kern-0.25emI}} %{\mathds{1}}
\newcommand\dsone{\mathbbm{1}}


\newcommand{\D}{\ensuremath{\mathbb{D}}}
\newcommand{\M}{\ensuremath{\mathbb{M}}}
\newcommand{\1}{\ensuremath{\mathbbm{1}}}
%------------------------------------------------------statistqiues
\DeclareMathOperator{\estMC}{\widehat \theta_n^{\,\,{\tt mc}}}
\DeclareMathOperator{\estMV}{\widehat \theta_n^{\,\,{\tt mv}}}
%\DeclareMathOperator{\est}{\widehat \theta_{\mathnormal{n}}}
\DeclareMathOperator{\var}{\mathrm{Var}}
\DeclareMathOperator{\Xbar}{\overline{\mathnormal{X}}_\mathnormal{n}}
%-----------------------------------------------------couleur
\newcommand{\blue}[1]{{\color{blue} #1}}
\newcommand{\green}[1]{{\color{green} #1}}
\newcommand{\red}[1]{{\color{red} #1}}%
%--------------------------------------nice circled with tikz
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}
\newcommand*\rect[1]{\tikz[baseline=(char.base)]{
            \node[shape=rectangle,draw,inner sep=2pt] (char) {#1};}}
%-----------------------------------------------------beamer
%\addtobeamertemplate{footline}{\insertframenumber/\inserttotalframenumber}% % insert page number

\newcommand \E{\mathbb{E}}
\newcommand \R{\mathbb{R}}
\newcommand \N{\mathbb{N}}
%----------------------------------------------------mathcal
\newcommand \cA{{\cal A}}
\newcommand \cB{{\cal B}}
\newcommand \cC{{\cal C}}
\newcommand \cD{{\cal D}}
\newcommand \cE{{\cal E}}
\newcommand \cF{{\cal F}}
\newcommand \cG{{\cal G}}
\newcommand \cH{{\cal H}}
\newcommand \cI{{\cal I}}
\newcommand \cJ{{\cal J}}
\newcommand \cK{{\cal K}}
\newcommand \cL{{\cal L}}
\newcommand \cM{{\cal M}}
\newcommand \cN{{\cal N}}
\newcommand \cO{{\cal O}}
\newcommand \cP{{\cal P}}
\newcommand \cQ{{\cal Q}}
\newcommand \cR{{\cal R}}
\newcommand \cS{{\cal S}}
\newcommand \cT{{\cal T}}
\newcommand \cU{{\cal U}}
\newcommand \cV{{\cal V}}
\newcommand \cW{{\cal W}}
\newcommand \cX{{\cal X}}
\newcommand \cY{{\cal Y}}
\newcommand \cZ{{\cal Z}}
%-------------------------------------------------mathbb
\newcommand \bA{{\mathbb A}}
\newcommand \bB{{\mathbb B}}
\newcommand \bC{{\mathbb C}}
\newcommand \bD{{\mathbb D}}
\newcommand \bE{{\mathbb E}}
\newcommand \bF{{\mathbb F}}
\newcommand \bG{{\mathbb G}}
\newcommand \bH{{\mathbb H}}
\newcommand \bI{{\mathbb I}}
\newcommand \bJ{{\mathbb J}}
\newcommand \bK{{\mathbb K}}
\newcommand \bL{{\mathbb L}}
\newcommand \bM{{\mathbb M}}
\newcommand \bN{{\mathbb N}}
\newcommand \bO{{\mathbb O}}
\newcommand \bP{{\mathbb P}}
\newcommand \bQ{{\mathbb Q}}
\newcommand \bR{{\mathbb R}}
\newcommand \bS{{\mathbb S}}
\newcommand \bT{{\mathbb T}}
\newcommand \bU{{\mathbb U}}
\newcommand \bV{{\mathbb V}}
\newcommand \bW{{\mathbb W}}
\newcommand \bX{{\mathbb X}}
\newcommand \bY{{\mathbb Y}}
\newcommand \bZ{{\mathbb Z}}
%-------------------------------------------------mathfrak
\newcommand \fA{{\mathfrak A}}
\newcommand \fB{{\mathfrak B}}
\newcommand \fC{{\mathfrak C}}
\newcommand \fD{{\mathfrak D}}
\newcommand \fE{{\mathfrak E}}
\newcommand \fF{{\mathfrak F}}
\newcommand \fG{{\mathfrak G}}
\newcommand \fH{{\mathfrak H}}
\newcommand \fI{{\mathfrak I}}
\newcommand \fJ{{\mathfrak J}}
\newcommand \fK{{\mathfrak K}}
\newcommand \fL{{\mathfrak L}}
\newcommand \fM{{\mathfrak M}}
\newcommand \fN{{\mathfrak N}}
\newcommand \fO{{\mathfrak O}}
\newcommand \fP{{\mathfrak P}}
\newcommand \fQ{{\mathfrak Q}}
\newcommand \fR{{\mathfrak R}}
\newcommand \fS{{\mathfrak S}}
\newcommand \fT{{\mathfrak T}}
\newcommand \fU{{\mathfrak U}}
\newcommand \fV{{\mathfrak V}}
\newcommand \fW{{\mathfrak W}}
\newcommand \fX{{\mathfrak X}}
\newcommand \fY{{\mathfrak Y}}
\newcommand \fZ{{\mathfrak Z}}
%------------------------------------------------- vectors (bold)
\newcommand{\vmu}{{\boldsymbol{\mu}}}
\newcommand{\vf}{{\mathbf{f}}}
\newcommand{\vtheta}{{\boldsymbol{\theta}}}
\newcommand{\vbeta}{{\boldsymbol{\beta}}}
\newcommand{\vc}{{\boldsymbol{1}}}
\newcommand{\vlambda}{{\boldsymbol{\lambda}}}
\newcommand{\vv}{{\boldsymbol{v}}}
\newcommand{\vh}{{\boldsymbol{h}}}
\newcommand{\ve}{{\boldsymbol{e}}}
\newcommand{\vzero}{{\boldsymbol{0}}}
\newcommand{\vx}{{\boldsymbol{x}}}
\newcommand{\vz}{{\boldsymbol{z}}}
\newcommand{\htheta}{{\boldsymbol{\hat \theta}}}
\newcommand{\vu}{{\boldsymbol{u}}}
\newcommand{\vw}{{\boldsymbol{w}}}
\newcommand{\vb}{{\boldsymbol{b}}}
\newcommand{\hmu}{\boldsymbol{\hat \mu}}
\newcommand{\tildemu}{{\boldsymbol{\tilde \mu}}}
\newcommand{\vy}{\mathbf{y}}
\newcommand{\vxi}{{\boldsymbol{\xi}}}
\newcommand{\vg}{{\boldsymbol{g}}}
\newcommand{\vdelta}{{\boldsymbol{\delta}}}
%---------------------------------------------hat letters
\newcommand{\hM}{\hat f}
\newcommand{\hrho}{\hat \rho}


==> packages_notes.tex <==
\setlength{\textwidth}{7in}
\setlength{\marginparwidth}{-0.5in}
\setlength{\hoffset}{-0.2in}
\setlength{\oddsidemargin}{-0.1in}
\setlength{\voffset}{-0.8in}
\setlength{\textheight}{690pt}

\usepackage{natbib}
\usepackage{graphicx}
\usepackage{color}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amscd}
\usepackage{bbm}
\usepackage{tikz}
\usepackage{hyperref}
\hypersetup{
    bookmarks=true,         % show bookmarks bar?
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=red,          % color of internal links (change box color with linkbordercolor)
    citecolor=green,        % color of links to bibliography
    filecolor=magenta,      % color of file links
    urlcolor=cyan           % color of external links
}
%\usepackage{showkeys}

\usepackage[utf8]{inputenc}
%\usepackage[T1]{fontenc}

%\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{bbm} %indicatrice
%\usepackage{caption}
%\usepackage{fullpage}
%\usepackage{lmodern}
%\usepackage{fourier}
%\usepackage{comment}
%\usepackage{pict2e}
\usepackage{algorithm}
\usepackage{algorithmic}
%\usepackage[small,nohug,heads=vee]{diagrams} 

%\usepackage{mathrsfs}
%\usepackage{geometry}	
%\geometry{hmargin=2.5cm,vmargin=3cm}
%\usepackage[utopia]{mathdesign}

\usepackage{marginnote}
\newcommand{\bluenote}[1]{ {\color{blue} #1}  \marginnote{({\color{blue} G-note})}}
\newcommand{\greennote}[1]{{\color{teal} #1}  \marginnote{({\color{teal} P-note})}}
\newcommand{\rednote}[1]{  {\color{red} #1}   \marginnote{({\color{red} V-note})}}


\newtheorem{Theorem}{Theorem}
\newtheorem{Assumption}{Assumption}
\newtheorem{Definition}{Definition}
\newtheorem{Lemma}{Lemma}
\newtheorem{Proposition}{Proposition}
\newtheorem{Corollary}{Corollary}
\newtheorem{Remark}{Remark}

%\allowdisplaybreaks


